An in silico-based review on anisotropic hyperelastic constitutive models for soft biological tissues

We review nine invariant and dispersion-type anisotropic hyperelastic constitutive models for soft biological tissues based on their fitting performance to experimental data from three different human tissues. For this, we used a hybrid multi-objective optimization procedure. A genetic algorithm is devised to generate the initial guesses followed by a gradient-based search algorithm. The constitutive models are then fit to a set of uniaxial and biaxial tension experiments conducted on tissues with differing fiber orientations. For the in silico investigation, experiments conducted on aneurysmatic abdominal aorta, linea alba, and rectus sheath tissues are utilized. Accordingly, the models are ranked with respect to an objec tive normalized quality of fit metric. Finally, a detailed discussion is carried out on the fitting performance of each model. This work provides a valuable quantitative comparison of various anisotropic hyperelastic models, the findings of which can aid those modeling the behavior of soft tissues in selecting the best constitutive model for their particular application.

==> FIGs/DeformationModes/fig.tex <==
\begin{figure*}[th!]
\centering
{
  %
 \psfrag{1}[c][c] {1}
 \psfrag{a\)}[c][c] {(a)}
 \psfrag{b\)}[c][c] {(b)}
 \psfrag{c\)}[c][c] {(c)}
 \psfrag{d\)}[c][c] {d)}
 \psfrag{e\)}[c][c] {e)}
 \psfrag{f\)}[c][c] {f)}
 \psfrag{e1}[l][l] {$\Be_1$}
 \psfrag{e2}[c][c] {$\Be_2$}
 \psfrag{lambda}[l][l] {$\lambda$} 
 \psfrag{lambda1}[c][c] {$\lambda_{1}$}
 \psfrag{lambda2}[c][c] {$\lambda_{2}$}
 \includegraphics[width = 1.0\textwidth]{deformation_modes}}
\caption{Deformation modes: (a) uniaxial tension in $\Be_1$, (b) uniaxial tension in in $\Be_2$, and (c) equibiaxial tension.}
\label{def-modes}
\end{figure*}


==> FIGs/bivariate-dispersion/fig.tex <==
 \begin{figure*}[tb!]%
  \normalsize{
\centering%
{
{
\psfrag{bb}    [c][c] {$a$}%
\psfrag{xx}    [c][c] {$b$}%
\psfrag{yy}    [c][c] {$\kappa_{op}$}%
\psfrag{yyy}    [c][c] {$\kappa_{ip}$}%
%
\psfrag{a\)}    [r][r] {(a)}%
\psfrag{b\)}    [r][r] {(b)}%
\psfrag{ 20}     [c][c] {$20$}%
\psfrag{ 15}     [c][c] {$15$}%
\psfrag{ 10}       [c][c] {$10$}%
\psfrag{ 5}       [c][c] {$5$}%
\psfrag{ 0}       [c][c] {$0$}%
%%
\psfrag{ 0.25}  [r][r] {$0.25$}%
\psfrag{ 0.3}    [r][r] {$0.3$}%
\psfrag{ 0.35}  [r][r] {$0.35$}%
\psfrag{ 0.4}    [r][r] {$0.4 $}%
\psfrag{ 0.45}  [r][r] {$0.45$}%
\psfrag{ 0.5}  [r][r] {$0.5$}%
\psfrag{ 0.75}  [r][r] {$0.75$}%
\psfrag{ 1}  [r][r] {$1$}%
%
\psfrag{-20}     [c][c] {$-20$}%
\psfrag{-15}     [c][c] {$-15$}%
\psfrag{-10}       [c][c] {$-10$}%
\psfrag{-5}       [c][c] {$-5$}%
\psfrag{ 0}       [c][c] {$0$}%
%
\includegraphics[width = 1\textwidth]{bivariate.eps}}}%
\caption{(a) Relation between the dispersion parameter $\kappa_{op}$ and the out-of-plane concentration parameter $b$ of von-Mises distribution and (b) relation between the dispersion parameter $\kappa_{ip}$ and the in-plane concentration parameter $a$ of von-Mises distribution.}}
\label{bivariate}%
\end{figure*}%
%==============================


==> FIGs/dispersionparameterGasser/fig.tex <==
\begin{figure*}[thb!]%
\centering%
{
{
\psfrag{bb}    [c][c] {\large{b}}%
\psfrag{yyy}    [c][c] {\large{$\kappa$}}%
%
\psfrag{ 20}     [c][c] {\normalsize{$20$}}%
\psfrag{ 15}     [c][c] {\normalsize{$15$}}%
\psfrag{ 10}       [c][c] {\normalsize{$10$}}%
\psfrag{ 5}       [c][c] {\normalsize{$5$}}%
\psfrag{ 0}       [c][c] {\normalsize{$0$}}%
%%
\psfrag{ 0.4}    [r][r] {\normalsize{$0.4$}}%
\psfrag{ 0.3}    [r][r] {\normalsize{$0.3$}}%
\psfrag{ 0.2}  [r][r] {\normalsize{$0.2$}}%
\psfrag{ 0.1}    [r][r] {\normalsize{$0.1$}}%
\psfrag{ 0}    [r][r] {\normalsize{$0$}}%
%%
\psfrag{ 20}     [c][c] {\normalsize{$20$}}%
\psfrag{ 16}     [c][c] {\normalsize{$12$}}%
\psfrag{ 12}     [c][c] {\normalsize{$12$}}%
\psfrag{ 8}     [c][c] {\normalsize{$8$}}%
\psfrag{ 4}     [c][c] {\normalsize{$4$}}%
%%
\psfrag{-1.5708}     [c][c] {\normalsize{$-\pi/2$}}%
\psfrag{ 1.5708}     [c][c] {\normalsize{$\pi/2$}}%
\psfrag{-0.785398}     [c][c] {\normalsize{$-\pi/4$}}%
\psfrag{ 0.785398}     [c][c] {\normalsize{$\pi/4$}}%
%
\psfrag{xx}    [c][c] {\large{$\Theta$}}%
\psfrag{yy}    [c][c] {\large{$\rho$ }}%
%
\psfrag{b1}    [l][l] {\normalsize{$b=1$}}%
\psfrag{b2}    [l][l] {\normalsize{$b=2$}}%
\psfrag{b3}    [l][l] {\normalsize{$b=3$}}%

\psfrag{a\)}    [r][r] {(a)}%
\psfrag{b\)}    [r][r] {(b)}%


%
%
\includegraphics[width=0.95\textwidth]{measure-dispersion.eps}}}%
\caption{(a) Graphical representation of the von-Mises distribution of collagen fibers and (b) relation between the dispersion parameter $\kappa$ and the concentration parameter of the von-Mises distribution.}
\label{measure-dispersion}%s
\end{figure*}%



==> FIGs/isoinv/fig.tex <==
\begin{figure*}[!htbp]
\begin{center}
\psfrag{a}  [l][l]  {(a)}
\psfrag{b}  [l][l]  {(b)}
\psfrag{c}  [l][l]  {(c)}

\psfrag{e1} [r][r]{$\Be_1$}
\psfrag{e2} [l][l]{$\Be_2$}
\psfrag{e3} [l][l]{$\Be_3$}
\psfrag{a0} [c][c]{$a_0$}
%------------------------8ch-1.eps--------------------
\psfrag{x1} [l][l] {$\BN^1$}
\psfrag{x2} [l][l] {$\BN^2$}
\psfrag{x3} [l][l] { $\BN^3$}
%
\psfrag{l1} [c][c] { $\lambda_1a_0$}
\psfrag{l2} [c][c] { $\lambda_2 a_0$}
\psfrag{l3} [r][r] { $\lambda_3 a_0$}
\psfrag{a1} [c][c] { $\nu_2 a^2_0$}
\psfrag{a2} [c][c] { $\nu_1 a^2_0$}
\psfrag{a3} [c][c] { $\nu_3 a^2_0$}
%
\psfrag{rr} [c][c] { $\lambda r_0$}
\includegraphics[width=0.9\textwidth]{mean-def1}
\caption{The invariants (a) $I_1(\BC)=\lambda_1^2+\lambda_2^2+\lambda_3^2$ as the sum of squares of the principal stretches, (b)  $I_2(\BC)= \nu_1^2+\nu_2^2+\nu_3^2$  as the sum of squares of principal areal stretches, where $\nu_i=J/\lambda_i$, and (c) $I_3=J^2=\lambda_1^2\lambda_2^2\lambda_3^2$ as the square of the volumetric stretch.}
\label{isoinv}
\end{center}
\end{figure*}
%==============================


==> FIGs/polarplotforinv/hgo/fig.tex <==
 \begin{figure*}[h!]%
\centering%
{
{
\psfrag{x}    [c][c] {\scriptsize{(a)}}%
\psfrag{y}    [c][c] {\scriptsize{(b)}}%
\psfrag{z}    [c][c] {\scriptsize{(c)}}%
\psfrag{HGO model}    [c][c] { }%
\psfrag{a}    [c][c] {\scriptsize{$1.5$}}%


\psfrag{0}    [l][l] {\footnotesize{$0^{\circ}$}}
\psfrag{30}    [l][l] {\footnotesize{$30^{\circ}$}}
\psfrag{60}    [l][l] {\footnotesize{$60^{\circ}$}}
\psfrag{90}    [c][c] {\footnotesize{$90^{\circ}$}}
\psfrag{120}    [r][r] {\footnotesize{$120^{\circ}$}}
\psfrag{150}    [r][r] {\footnotesize{$150^{\circ}$}}
\psfrag{180}    [c][c] {\footnotesize{$180^{\circ}$}}
\psfrag{210}    [r][r] {\footnotesize{$210^{\circ}$}}
\psfrag{240}    [r][r] {\footnotesize{$240^{\circ}$}}
\psfrag{270}    [c][c] {\footnotesize{$270^{\circ}$}}
\psfrag{300}    [l][l] {\footnotesize{$300^{\circ}$}}
\psfrag{330}    [l][l] {\footnotesize{$330^{\circ}$}}

\psfrag{0.3}    [c][c] {\footnotesize{$0.3$}}%
\psfrag{0.6}    [c][c] {\footnotesize{$0.6$}}%
\psfrag{0.9}    [c][c] {\footnotesize{$0.9$}}%

\psfrag{0.2}    [c][c] {\footnotesize{$0.2$}}%
\psfrag{0.4}    [c][c] {\footnotesize{$0.4$}}%


\psfrag{3}    [c][c] {\footnotesize{$3$}}%
\psfrag{6}    [c][c] {\footnotesize{$6$}}%
\psfrag{9}    [c][c] {\footnotesize{$9$}}%

\includegraphics[width = 1\textwidth]{hgo_polar.eps}}}%
\caption{The polar plots of the directional stiffness (DS) for the HGO model~\cite{holzapfel2000}; (a) two families of fibers distribution based on ET dataset for AAA tissue~\cite{niestrawska2016}, (b) one family of fibers distribution based on UT dataset for the linea alba~\cite{cooney2016}, (c) one family of fibers distribution based on UT datset for the rectus sheath~\cite{Martins2012}.}
\label{hgo-polar}
\end{figure*}%




==> FIGs/polarplotforinv/hsgr/fig.tex <==
 \begin{figure*}[h!]%
\centering%
{
{
\psfrag{x}    [c][c] {\scriptsize{(a)}}%
\psfrag{y}    [c][c] {\scriptsize{(b)}}%
\psfrag{z}    [c][c] {\scriptsize{(c)}}%
\psfrag{HGO model}    [c][c] { }%

\psfrag{0}    [l][l] {\footnotesize{$0^{\circ}$}}
\psfrag{30}    [l][l] {\footnotesize{$30^{\circ}$}}
\psfrag{60}    [l][l] {\footnotesize{$60^{\circ}$}}
\psfrag{90}    [c][c] {\footnotesize{$90^{\circ}$}}
\psfrag{120}    [r][r] {\footnotesize{$120^{\circ}$}}
\psfrag{150}    [r][r] {\footnotesize{$150^{\circ}$}}
\psfrag{180}    [c][c] {\footnotesize{$180^{\circ}$}}
\psfrag{210}    [r][r] {\footnotesize{$210^{\circ}$}}
\psfrag{240}    [r][r] {\footnotesize{$240^{\circ}$}}
\psfrag{270}    [c][c] {\footnotesize{$270^{\circ}$}}
\psfrag{300}    [l][l] {\footnotesize{$300^{\circ}$}}
\psfrag{330}    [l][l] {\footnotesize{$330^{\circ}$}}


\psfrag{0.01}    [c][c] {\footnotesize{$0.01$}}%
\psfrag{0.02}    [c][c] {\footnotesize{$0.02$}}%
\psfrag{0.03}    [c][c] {\footnotesize{$0.03$}}%

\psfrag{0.3}    [c][c] {\footnotesize{$0.2$}}%
\psfrag{0.6}    [c][c] {\footnotesize{$0.6$}}%
\psfrag{0.9}    [c][c] {\footnotesize{$0.9$}}%


\psfrag{0.005}    [c][c] {\footnotesize{$0.05$}}%
\psfrag{0.01}    [c][c] {\footnotesize{$0.01$}}%
\psfrag{0.015}    [c][c] {\footnotesize{$0.015$}}%

\includegraphics[width = 1\textwidth]{hsgr_polar.eps}}}%
\caption{The polar plots of the directional stiffness (DS) for the HSGR model~\cite{Holzapfel2005}; (a) two families of fibers distribution based on ET dataset for AAA tissue~\cite{niestrawska2016}, (b) one family of fibers distribution based on UT dataset for the linea alba~\cite{cooney2016}, (c) one family of fibers distribution based on UT datset for the rectus sheath~\cite{Martins2012}.}
\label{hsgr-polar}
\end{figure*}%




==> FIGs/polarplotforinv/ny/fig.tex <==
 \begin{figure*}[h!]%
\centering%
{
{
\psfrag{x}    [c][c] {\scriptsize{(a)}}%
\psfrag{y}    [c][c] {\scriptsize{(b)}}%
\psfrag{z}    [c][c] {\scriptsize{(c)}}%
%\psfrag{HGO model}    [c][c] { }%
\psfrag{0.2}    [c][c] { }%
\psfrag{0.4}    [c][c] { }%
\psfrag{0.6}    [c][c] { }%
\psfrag{3}    [c][c] { }%

\psfrag{0}    [l][l] {\footnotesize{$0^{\circ}$}}
\psfrag{30}    [l][l] {\footnotesize{$30^{\circ}$}}
\psfrag{60}    [l][l] {\footnotesize{$60^{\circ}$}}
\psfrag{90}    [c][c] {\footnotesize{$90^{\circ}$}}
\psfrag{120}    [r][r] {\footnotesize{$120^{\circ}$}}
\psfrag{150}    [r][r] {\footnotesize{$150^{\circ}$}}
\psfrag{180}    [c][c] {\footnotesize{$180^{\circ}$}}
\psfrag{210}    [r][r] {\footnotesize{$210^{\circ}$}}
\psfrag{240}    [r][r] {\footnotesize{$240^{\circ}$}}
\psfrag{270}    [c][c] {\footnotesize{$270^{\circ}$}}
\psfrag{300}    [l][l] {\footnotesize{$300^{\circ}$}}
\psfrag{330}    [l][l] {\footnotesize{$330^{\circ}$}}

\psfrag{0.3}    [c][c] {\footnotesize{$0.3$}}%
\psfrag{0.6}    [c][c] {\footnotesize{$0.6$}}%
\psfrag{0.9}    [c][c] {\footnotesize{$0.9$}}%

\psfrag{0.2}    [c][c] {\footnotesize{$0.2$}}%
\psfrag{0.4}    [c][c] {\footnotesize{$0.4$}}%
\psfrag{0.6}    [c][c] {\footnotesize{$0.6$}}%

\psfrag{3}    [c][c] {\footnotesize{$3$}}%
\psfrag{6}    [c][c] {\footnotesize{$6$}}%
\psfrag{9}    [c][c] {\footnotesize{$9$}}%

\includegraphics[width = 1\textwidth]{ny_polar.eps}}}%
\caption{The polar plots of the directional stiffness (DS) for the NY model~\cite{Newman1998}; (a) two families of fibers distribution based on ET dataset for AAA tissue~\cite{niestrawska2016}, (b) one family of fibers distribution based on UT dataset for the linea alba~\cite{cooney2016}, (c) one family of fibers distribution based on UT datset for the rectus sheath~\cite{Martins2012}.}
\label{ny-polar}
\end{figure*}%




==> FIGs/polarplotforinv/os/fig.tex <==
 \begin{figure*}[h!]%
\centering%
{
{
\psfrag{x}    [c][c] {\scriptsize{(a)}}%
\psfrag{y}    [c][c] {\scriptsize{(b)}}%
\psfrag{z}    [c][c] {\scriptsize{(c)}}%
%\psfrag{HGO model}    [c][c] { }%


\psfrag{0}    [l][l] {\footnotesize{$0^{\circ}$}}
\psfrag{30}    [l][l] {\footnotesize{$30^{\circ}$}}
\psfrag{60}    [l][l] {\footnotesize{$60^{\circ}$}}
\psfrag{90}    [c][c] {\footnotesize{$90^{\circ}$}}
\psfrag{120}    [r][r] {\footnotesize{$120^{\circ}$}}
\psfrag{150}    [r][r] {\footnotesize{$150^{\circ}$}}
\psfrag{180}    [c][c] {\footnotesize{$180^{\circ}$}}
\psfrag{210}    [r][r] {\footnotesize{$210^{\circ}$}}
\psfrag{240}    [r][r] {\footnotesize{$240^{\circ}$}}
\psfrag{270}    [c][c] {\footnotesize{$270^{\circ}$}}
\psfrag{300}    [l][l] {\footnotesize{$300^{\circ}$}}
\psfrag{330}    [l][l] {\footnotesize{$330^{\circ}$}}

\psfrag{0.2}    [c][c] {\footnotesize{$0.2$}}%
\psfrag{0.4}    [c][c] {\footnotesize{$0.4$}}%
\psfrag{0.6}    [c][c] {\footnotesize{$0.6$}}%

\psfrag{0.02}    [c][c] {\footnotesize{$0.02$}}%
\psfrag{0.04}    [c][c] {\footnotesize{$0.04$}}%
\psfrag{0.06}    [c][c] {\footnotesize{$0.06$}}%

\psfrag{1}    [c][c] {\footnotesize{$1$}}%
\psfrag{2}    [c][c] {\footnotesize{$2$}}%
\psfrag{3}    [c][c] {\footnotesize{$3$}}%


\includegraphics[width = 1\textwidth]{os_polar.eps}}}%
\caption{The polar plots of the directional stiffness (DS) for the OS model~\cite{Ogden2007}; (a) two families of fibers distribution based on ET dataset for AAA tissue~\cite{niestrawska2016}, (b) one family of fibers distribution based on UT dataset for the linea alba~\cite{cooney2016}, (c) one family of fibers distribution based on UT datset for the rectus sheath~\cite{Martins2012}.}
\label{os-polar}
\end{figure*}%




==> FIGs/polarplots/amdm_polar/fig.tex <==
 \begin{figure*}[tb!]%
\centering%
{
{
\psfrag{a}    [c][c] {\scriptsize{(a)}}%
\psfrag{b}    [c][c] {\scriptsize{(b)}}%
\psfrag{c}    [c][c] {\scriptsize{(c)}}%

\psfrag{0}    [l][l] {\footnotesize{$0^{\circ}$}}
\psfrag{30}    [l][l] {\footnotesize{$30^{\circ}$}}
\psfrag{60}    [l][l] {\footnotesize{$60^{\circ}$}}
\psfrag{90}    [c][c] {\footnotesize{$90^{\circ}$}}
\psfrag{120}    [r][r] {\footnotesize{$120^{\circ}$}}
\psfrag{150}    [r][r] {\footnotesize{$150^{\circ}$}}
\psfrag{180}    [c][c] {\footnotesize{$180^{\circ}$}}
\psfrag{210}    [r][r] {\footnotesize{$210^{\circ}$}}
\psfrag{240}    [r][r] {\footnotesize{$240^{\circ}$}}
\psfrag{270}    [c][c] {\footnotesize{$270^{\circ}$}}
\psfrag{300}    [l][l] {\footnotesize{$300^{\circ}$}}
\psfrag{330}    [l][l] {\footnotesize{$330^{\circ}$}}


%\psfrag{1}    [c][c] {\footnotesize{$1$}}%
%\psfrag{2}    [c][c] {\footnotesize{$2$}}%
%\psfrag{3}    [c][c] {\footnotesize{$3$}}%

\includegraphics[width = 1\textwidth]{amdm_polar.eps}}}%
\caption{The polar plots of the density distribution (DD) and the directional stiffness (DS) for the AMDM model~\cite{Alastrue2009}; (a) two families of fibers distribution based on ET dataset for AAA tissue~\cite{niestrawska2016}, (b) one family of fibers distribution based on UT dataset for the linea alba~\cite{cooney2016}, (c) one family of fibers distribution based on UT dataset for the rectus sheath~\cite{Martins2012}.}
\label{amdm-polar}
\end{figure*}%




==> FIGs/polarplots/asmd_polar/fig.tex <==
 \begin{figure*}[tb!]%
\centering%
{
{
\psfrag{a}    [c][c] {\scriptsize{(a)}}%
\psfrag{b}    [c][c] {\scriptsize{(b)}}%
\psfrag{c}    [c][c] {\scriptsize{(c)}}%

\psfrag{0}    [l][l] {\footnotesize{$0^{\circ}$}}
\psfrag{30}    [l][l] {\footnotesize{$30^{\circ}$}}
\psfrag{60}    [l][l] {\footnotesize{$60^{\circ}$}}
\psfrag{90}    [c][c] {\footnotesize{$90^{\circ}$}}
\psfrag{120}    [r][r] {\footnotesize{$120^{\circ}$}}
\psfrag{150}    [r][r] {\footnotesize{$150^{\circ}$}}
\psfrag{180}    [c][c] {\footnotesize{$180^{\circ}$}}
\psfrag{210}    [r][r] {\footnotesize{$210^{\circ}$}}
\psfrag{240}    [r][r] {\footnotesize{$240^{\circ}$}}
\psfrag{270}    [c][c] {\footnotesize{$270^{\circ}$}}
\psfrag{300}    [l][l] {\footnotesize{$300^{\circ}$}}
\psfrag{330}    [l][l] {\footnotesize{$330^{\circ}$}}


\psfrag{1}    [c][c] {\footnotesize{$1$}}%
\psfrag{2}    [c][c] {\footnotesize{$2$}}%
\psfrag{3}    [c][c] {\footnotesize{$3$}}%

\includegraphics[width = 1\textwidth]{asmd_polar.eps}}}%
\caption{The polar plots of the density distribution (DD) and the directional stiffness (DS) for the ASMD model~\cite{Alastrue2010}; (a) two families of fibers distribution based on ET dataset for AAA tissue~\cite{niestrawska2016}, (b) one family of fibers distribution based on UT dataset for the linea alba~\cite{cooney2016}, (c) one family of fibers distribution based on UT dataset for the rectus sheath~\cite{Martins2012}.}
\label{asmd-polar}
\end{figure*}%




==> FIGs/polarplots/dbb_polar/fig.tex <==
 \begin{figure*}[tb!]%
\centering%
{
{
\psfrag{a}    [c][c] {\scriptsize{(a)}}%
\psfrag{b}    [c][c] {\scriptsize{(b)}}%
\psfrag{c}    [c][c] {\scriptsize{(c)}}%
%\psfrag{x1}    [l][l] {\footnotesize{DS for the 1$^{st}$ family}}%
%\psfrag{x2}    [l][l] {\footnotesize{DS for the 2$^{nd}$ family}}%
\psfrag{0}    [l][l] {\footnotesize{$0^{\circ}$}}
\psfrag{30}    [l][l] {\footnotesize{$30^{\circ}$}}
\psfrag{60}    [l][l] {\footnotesize{$60^{\circ}$}}
\psfrag{90}    [c][c] {\footnotesize{$90^{\circ}$}}
\psfrag{120}    [r][r] {\footnotesize{$120^{\circ}$}}
\psfrag{150}    [r][r] {\footnotesize{$150^{\circ}$}}
\psfrag{180}    [c][c] {\footnotesize{$180^{\circ}$}}
\psfrag{210}    [r][r] {\footnotesize{$210^{\circ}$}}
\psfrag{240}    [r][r] {\footnotesize{$240^{\circ}$}}
\psfrag{270}    [c][c] {\footnotesize{$270^{\circ}$}}
\psfrag{300}    [l][l] {\footnotesize{$300^{\circ}$}}
\psfrag{330}    [l][l] {\footnotesize{$330^{\circ}$}}


\psfrag{1}    [c][c] {\footnotesize{$1$}}%
\psfrag{2}    [c][c] {\footnotesize{$2$}}%
\psfrag{3}    [c][c] {\footnotesize{$3$}}%

\includegraphics[width = 1\textwidth]{dbb_polar.eps}}}%
\caption{The polar plots of the density distribution (DD) and the directional stiffness (DS) for the DBB model~\cite{Driessen2005}; (a) two families of fibers distribution based on ET dataset for AAA tissue~\cite{niestrawska2016}, (b) one family of fibers distribution based on UT dataset for the linea alba~\cite{cooney2016}, (c) one family of fibers distribution based on UT dataset for the rectus sheath~\cite{Martins2012}.}
\label{dbb-polar}
\end{figure*}%




==> FIGs/polarplots/goh_polar/fig.tex <==
 \begin{figure*}[th!]%
\centering%
{
{
\psfrag{a}    [c][c] {\scriptsize{(a)}}%
\psfrag{b}    [c][c] {\scriptsize{(b)}}%
\psfrag{c}    [c][c] {\scriptsize{(c)}}%

\psfrag{0}    [l][l] {\footnotesize{$0^{\circ}$}}
\psfrag{30}    [l][l] {\footnotesize{$30^{\circ}$}}
\psfrag{60}    [l][l] {\footnotesize{$60^{\circ}$}}
\psfrag{90}    [c][c] {\footnotesize{$90^{\circ}$}}
\psfrag{120}    [r][r] {\footnotesize{$120^{\circ}$}}
\psfrag{150}    [r][r] {\footnotesize{$150^{\circ}$}}
\psfrag{180}    [c][c] {\footnotesize{$180^{\circ}$}}
\psfrag{210}    [r][r] {\footnotesize{$210^{\circ}$}}
\psfrag{240}    [r][r] {\footnotesize{$240^{\circ}$}}
\psfrag{270}    [c][c] {\footnotesize{$270^{\circ}$}}
\psfrag{300}    [l][l] {\footnotesize{$300^{\circ}$}}
\psfrag{330}    [l][l] {\footnotesize{$330^{\circ}$}}


\psfrag{1}    [c][c] {\footnotesize{$1$}}%
\psfrag{2}    [c][c] {\footnotesize{$2$}}%
\psfrag{3}    [c][c] {\footnotesize{$3$}}%

\includegraphics[width = 1\textwidth]{goh_polar.eps}}}%
\caption{The polar plots of the density distribution (DD) and the directional stiffnesses (DS) for the GOH model~\cite{Gasser2006}; (a) two families of fibers distribution based on ET dataset for AAA tissue~\cite{niestrawska2016}, (b) one family of fibers distribution based on UT dataset for the linea alba~\cite{cooney2016}, (c) one family of fibers distribution based on UT dataset for the rectus sheath~\cite{Martins2012}.}
\label{goh-polar}
\end{figure*}%




==> FIGs/polarplots/hnors_polar/fig.tex <==
 \begin{figure*}[thb!]%
\centering%
{
{
\psfrag{a}    [c][c] {\scriptsize{(a)}}%
\psfrag{b}    [c][c] {\scriptsize{(b)}}%
\psfrag{c}    [c][c] {\scriptsize{(c)}}%
\psfrag{d}    [c][c] {\scriptsize{(d)}}%
\psfrag{e}    [c][c] {\scriptsize{(e)}}%
\psfrag{f}    [c][c] {\scriptsize{(f)}}%

\psfrag{0}    [c][c] {\footnotesize{$0^{\circ}$}}
\psfrag{30}    [l][l] {\footnotesize{$30^{\circ}$}}
\psfrag{60}    [l][l] {\footnotesize{$60^{\circ}$}}
\psfrag{90}    [l][l] {\footnotesize{$90^{\circ}$}}
\psfrag{120}    [l][l] {\footnotesize{$120^{\circ}$}}
\psfrag{150}    [l][l] {\footnotesize{$150^{\circ}$}}
\psfrag{180}    [l][l] {\footnotesize{$180^{\circ}$}}
\psfrag{210}    [l][l] {\footnotesize{$210^{\circ}$}}
\psfrag{240}    [l][l] {\footnotesize{$240^{\circ}$}}
\psfrag{270}    [l][l] {\footnotesize{$270^{\circ}$}}
\psfrag{300}    [l][l] {\footnotesize{$300^{\circ}$}}
\psfrag{330}    [l][l] {\footnotesize{$330^{\circ}$}}
\includegraphics[width = 1\textwidth]{hnors_polar.eps}}}%
\caption{The polar plots of density distribution (DD) and the directional stiffness (DS) for the HNORS model~\cite{Holzapfel2015b}; (a) in-plane distribution of two families of fibers based on ET dataset for AAA tissue~\cite{niestrawska2016}, (b) out-of-plane distribution of one families of fibers based on ET dataset for AAA tissue~\cite{niestrawska2016} (c) in-plane distribution of one family of fibers based on UT dataset for the linea alba~\cite{cooney2016}, (d) out-of-plane distribution of one family of fibers based on UT dataset for the linea alba~\cite{cooney2016}, (e) in-plane distribution of one family of fibers based on UT dataset for the rectus sheath~\cite{Martins2012}, (f) out-of-plane distribution of one family of fibers based on UT dataset for the rectus sheath~\cite{Martins2012}.}
\label{hnors-polar}
\end{figure*}%




==> FIGs/results_new/AAA/fig.tex <==
 \begin{figure*}[thb!]%
%\centering%
%{
%{
\psfrag{xx}    [c][c] {\scriptsize{$\lambda$}}%
\psfrag{yy}    [c][c] {\scriptsize{$\textrm{P}~\textrm{[kPa]}$}}%
\psfrag{e}[c][c] {\footnotesize{$P_{11}^{exp}$}}
\psfrag{ee}[c][c] {\footnotesize{$P_{22}^{exp}$}}
\psfrag{m}[c][c] {\footnotesize{$P_{11}$}}
\psfrag{mm}[c][c] {\footnotesize{$P_{22}$}}
%
%
\psfrag{T1}      [l][r]  {\scriptsize{$\text{ET data points}$}}%
\psfrag{T2}      [l][r]  {\scriptsize{$\text{ET model fit}$}}%
\psfrag{a\)}     [r][r]{\scriptsize{$\text{a)}$}}%
\psfrag{b\)}     [r][r]{\scriptsize{$\text{b)}$}}%
\psfrag{c\)}     [r][r]{\scriptsize{$\text{c)}$}}%
\psfrag{d\)}     [r][r]{\scriptsize{$\text{d)}$}}%
\psfrag{e\)}     [r][r]{\scriptsize{$\text{e)}$}}%
\psfrag{f\)}     [r][r]{\scriptsize{$\text{f)}$}}%
\psfrag{g\)}     [r][r]{\scriptsize{$\text{g)}$}}%
\psfrag{h\)}     [r][r]{\scriptsize{$\text{h)}$}}%
\psfrag{i\)}     [r][r]{\scriptsize{$\text{i)}$}}%

%
\psfrag{ 1}       [c][c] {\footnotesize{$1$}}%%
\psfrag{ 1.04}     [c][c] {\footnotesize{$1.04$}}%
\psfrag{ 1.08}     [c][c] {\footnotesize{$1.08$}}%
\psfrag{ 1.12}     [c][c] {\footnotesize{$1.12$}}%
\psfrag{ 1.16}     [c][c] {\footnotesize{$1.16$}}%
%%
\psfrag{ 50}    [r][r] {\footnotesize{$60$}}%
\psfrag{ 40}    [r][r] {\footnotesize{$45$}}%
\psfrag{ 30}    [r][r] {\footnotesize{$30$}}%
\psfrag{ 20}   [r][r] {\footnotesize{$20$}}%
\psfrag{ 10}    [r][r] {\footnotesize{$10$}}%
\psfrag{ 0}      [r][r] {\footnotesize{$0$}}%
%
%
\includegraphics[width = 1.06\textwidth]{aaa.eps}%
%\caption{ASMD model~\cite{Alastrue2010} predictions for i) ET dataset for AAA tissue~\cite{niestrawska2016}, ii) UT dataset for linea alba~\cite{cooney2016}, iii) UT dataset for rectus sheath~\cite{Martins2012}.}
\caption{a) NY model~\cite{Newman1998}, b) HGO model~\cite{holzapfel2000}, c) OS model~\cite{Ogden2007}, d) HSGR model~\cite{Holzapfel2005}, e) GOH model~\cite{Gasser2006}, f) HNORS  model~\cite{Holzapfel2015b}, g) DBB model~\cite{Driessen2005}, h) AMDM model~\cite{Alastrue2009}, i) ASMD model~\cite{Alastrue2010}  predictions for ET dataset for AAA tissue~\cite{niestrawska2016}.}
\label{aaa-plot}
\end{figure*}%



==> FIGs/results_new/LA/fig.tex <==
 \begin{figure*}[th!]%
\centering%
{
{
\psfrag{xx}    [c][c] {\scriptsize{$\lambda$}}%
\psfrag{yy}    [c][c] {\scriptsize{$\textrm{P}~\textrm{[MPa]}$}}%
\psfrag{e}[c][c] {\footnotesize{$P_{11}^{exp}$}}
\psfrag{ee}[c][c] {\footnotesize{$P_{22}^{exp}$}}
\psfrag{m}[c][c] {\footnotesize{$P_{11}$}}
\psfrag{mm}[c][c] {\footnotesize{$P_{22}$}}
%
%
\psfrag{a\)}     [r][r]{\scriptsize{$\text{a)}$}}%
\psfrag{b\)}    [r][r]{\scriptsize{$\text{b)}$}}%
\psfrag{c\)}    [r][r]{\scriptsize{$\text{c)}$}}%
\psfrag{d\)}     [r][r]{\scriptsize{$\text{d)}$}}%
\psfrag{e\)}    [r][r]{\scriptsize{$\text{e)}$}}%
\psfrag{f\)}    [r][r]{\scriptsize{$\text{f)}$}}%
\psfrag{g\)}     [r][r]{\scriptsize{$\text{g)}$}}%
\psfrag{h\)}    [r][r]{\scriptsize{$\text{h)}$}}%
\psfrag{i\)}    [r][r]{\scriptsize{$\text{i)}$}}%
%
\psfrag{ 1}       [c][c] {\footnotesize{$1$}}%%
\psfrag{ 1.04}     [r][r] {\footnotesize{$1.04$}}%
\psfrag{ 1.08}     [r][r] {\footnotesize{$1.08$}}%
\psfrag{ 1.12}     [r][r] {\footnotesize{$1.12$}}%
\psfrag{ 1.16}     [r][r] {\footnotesize{$1.16$}}%
\psfrag{ 1.2}     [c][c] {\footnotesize{$1.2$}}%
%%
\psfrag{ 5}    [r][r] {\footnotesize{$5$}}%
\psfrag{ 4}    [r][r] {\footnotesize{$4$}}%
\psfrag{ 3}    [r][r] {\footnotesize{$3$}}%
\psfrag{ 2}   [r][r] {\footnotesize{$2$}}%
\psfrag{ 1}    [r][r] {\footnotesize{$1$}}%
\psfrag{ 0}      [r][r] {\footnotesize{$0$}}%
%
%
\includegraphics[width = 1.06\textwidth]{la.eps}}}%
%\caption{ASMD model~\cite{Alastrue2010} predictions for i) ET dataset for AAA tissue~\cite{niestrawska2016}, ii) UT dataset for linea alba~\cite{cooney2016}, iii) UT dataset for rectus sheath~\cite{Martins2012}.}
\caption{a) NY model~\cite{Newman1998}, b) HGO model~\cite{holzapfel2000}, c) OS model~\cite{Ogden2007}, d) HSGR model~\cite{Holzapfel2005}, e) GOH model~\cite{Gasser2006}, f) HNORS  model~\cite{Holzapfel2015b}, g) DBB model~\cite{Driessen2005}, h) AMDM model~\cite{Alastrue2009}, i) ASMD model~\cite{Alastrue2010}  predictions for UT dataset for linea alba~\cite{cooney2016}.}
\label{la-plot}
\end{figure*}%



==> FIGs/results_new/RS/fig.tex <==
 \begin{figure*}[th!]%
\centering%
{
{
\psfrag{xx}    [c][c] {\scriptsize{$\lambda$}}%
\psfrag{yy}    [c][c] {\scriptsize{$\textrm{P}~\textrm{[MPa]}$}}%
\psfrag{e}[c][c] {\footnotesize{$P_{11}^{exp}$}}
\psfrag{ee}[c][c] {\footnotesize{$P_{22}^{exp}$}}
\psfrag{m}[c][c] {\footnotesize{$P_{11}$}}
\psfrag{mm}[c][c] {\footnotesize{$P_{22}$}}
%
%
\psfrag{a\)}     [r][r]{\scriptsize{$\text{a)}$}}%
\psfrag{b\)}    [r][r]{\scriptsize{$\text{b)}$}}%
\psfrag{c\)}    [r][r]{\scriptsize{$\text{c)}$}}%
\psfrag{d\)}     [r][r]{\scriptsize{$\text{d)}$}}%
\psfrag{e\)}    [r][r]{\scriptsize{$\text{e)}$}}%
\psfrag{f\)}    [r][r]{\scriptsize{$\text{f)}$}}%
\psfrag{g\)}     [r][r]{\scriptsize{$\text{g)}$}}%
\psfrag{h\)}    [r][r]{\scriptsize{$\text{h)}$}}%
\psfrag{i\)}    [r][r]{\scriptsize{$\text{i)}$}}%
%
%%
\psfrag{ 1}       [r][r] {\footnotesize{$1$}}%%
\psfrag{ 1.04}     [r][r] {\footnotesize{$1.04$}}%
\psfrag{ 1.08}     [c][c] {\footnotesize{$1.08$}}%
\psfrag{ 1.12}     [c][c] {\footnotesize{$1.12$}}%
\psfrag{ 1.16}     [l][l] {\footnotesize{$1.16$}}%
\psfrag{ 1.2}     [l][l] {\footnotesize{$1.2$}}%
%%
\psfrag{ 2}    [r][r] {\footnotesize{$2$}}%
\psfrag{ 1.5}    [r][r] {\footnotesize{$1.5$}}%
\psfrag{ 1}   [r][r] {\footnotesize{$1$}}%
\psfrag{ 0.5}    [r][r] {\footnotesize{$0.5$}}%
\psfrag{ 0}      [r][r] {\footnotesize{$0$}}%
%
%
\includegraphics[width = 1.06\textwidth]{rs.eps}}%
\caption{a) NY model~\cite{Newman1998}, b) HGO model~\cite{holzapfel2000}, c) OS model~\cite{Ogden2007}, d) HSGR model~\cite{Holzapfel2005}, e) GOH model~\cite{Gasser2006}, f) HNORS  model~\cite{Holzapfel2015b}, g) DBB model~\cite{Driessen2005}, h) AMDM model~\cite{Alastrue2009}, i) ASMD model~\cite{Alastrue2010}  predictions for UT dataset for rectus sheath~\cite{Martins2012}.}}
\label{rs-plot}
\end{figure*}%



==> FIGs/sphere/fig.tex <==
\begin{figure*}[th!]
    \scriptsize{
\psfrag{e1} [l][l]{ $\Be_1$}
\psfrag{e2} [r][r]{ $\Be_2$}
\psfrag{e3} [c][c]{ $\Be_3$}
\psfrag{phi}[c][c]{ $\phi$}
\psfrag{vphi}[c][c]{ $\theta$}
\psfrag{t}   [c][c]{ $\Bt$}
\psfrag{r}   [c][c]{ $\Br$}
\psfrag{dA}  [l][l]{ $dA$}
\psfrag{F}   [c][c]{$\bar\BF$}
\psfrag{lb}  [c][c]{ $\bar\lambda$}
\psfrag{l}   [c][c]{ $\lambda$}
\psfrag{S}   [l][l]{ $\SS$}
\psfrag{var}   [c][c]{$\vartheta$}
\psfrag{m1}   [c][c]{$\BM_1$}
\psfrag{m2}   [l][l]{$\BM_2$}
\psfrag{a}   [c][c]{(a)}
\psfrag{b}   [c][c]{(b)} 
\begin{center}
\includegraphics[width=0.9\textwidth]{twosphere.eps}%
\end{center}}
\caption {(a) The unit micro-sphere and the orientation vector, (b) mean fiber directions of two families of fiber lie on $\Be_1$-$\Be_2$ plane.}
\label{sphere}
\end{figure*}
%\caption {(a)The unit micro-sphere and the orientation vector $\Br = r_1 \Be_1 + r_2 \Be_2 + r_3 \Be_3$ where  $r_1 =\cos\Phi\sin\Theta$, $r_2=\sin\Phi\sin\Theta$ and $r_3=\cos\Theta$ in terms of spherical coordinates $\{\varphi,\vartheta \}$, respectively. (b) the unit sphere and unit orientation vectors for two families of fibers $\BM_1 = M_{1}^{(1)} \Be_1 + M_{1}^{(2)} \Be_2 + M_{1}^{(3)} \Be_3$ and $\BM_2 = M_{2}^{(1)} \Be_1 + M_{2}^{(2)} \Be_2 + M_{2}^{(3)} \Be_3$ where $M_{1}^{(1)}=\sin\vartheta$, $M_{1}^{(2)}=\cos\vartheta$, $M_{1}^{(3)}=0$, $M_{2}^{(1)}=-\sin\vartheta$, $M_{2}^{(2)}=\cos\vartheta$, $M_{2}^{(3)}=0$.}}




==> FIGs/threeFundamentalMaps/fig.tex <==
\begin{figure*}[!bthp]
\begin{center}
\psfrag{a}  [l][l]  {(a)}
\psfrag{b}  [l][l]  {(b)}
\psfrag{c}  [l][l]  {(c)}    
\psfrag{X}  [ct][ct]  {$  \BX $}
\psfrag{dX} [lb][lb]  {$ d\BX $}
\psfrag{dA} [rb][rb]  {$ d\BA $}
\psfrag{dV} [rb][rb]  {$ dV $}
\includegraphics[width=0.75\textwidth]{threefundmaps}
\caption{Three fundamental maps of a continuum: (a) The deformation gradient $\BF$ as a mapping of an infinitesimal line element, (b) its cofactor $\cof[\BF]$ as an area map, and (c) and its determinant $\det[\BF]$ as a volume map.}
\label{three-fund-maps}
\end{center}
%\vskip-6Ex
\end{figure*}
%==============================

